The skew spectrum of functions on finite groups and their homogeneous spaces

Whenever we have a group acting on a class of functions by translation, the bispectrum offers a principled and lossless way of representing such functions invariant to the action. Unfortunately, computing the bispectrum is often costly and complicated. In this paper we propose a unitarily equivalent, but easier to compute set of invariants, which we call the skew spectrum. For functions on homogeneous spaces the skew spectrum can be efficiently computed using some ideas from Clausen-type fast Fourier transforms.

==> background.tex <==
\section{Fourier transforms and the bispectrum}

In this paper \m{G} denotes a general finite group, and \m{\Rcal} denotes a complete set of inequivalent 
irreducible complex-valued matrix representations of \m{G}. 
Since \m{G} is finite, \m{\Rcal} is a finite set. 
We use the letter \m{\rho} to denote the individual representations, and \m{d_\rho} to denote their dimensionality. 
Hence, each \m{\rho\in\Rcal} is a homomorphism \m{\rho\colon G\to \CC^{d_\rho\times d_\rho}}.   
We assume that all representations are unitary, i.e., \m{\rho(x^{-1})=\br{\rho(x)}^{-1}=\rho(x)^\dag}. 
%, where \m{\mbox{}^\dag} denotes the conjugate transpose. 

We \marginpar{translation} denote the set of complex valued functions on \m{G} by \m{L(G)}. 
Given \m{f\in L(G)} and a group element \m{t}, the \df{left-translate} of \m{f} by \m{t} is the function 
\m{f^t\in L(G)} defined \m{f^t(x)=f(t^{-1}x)}. 
A functional \m{p\colon f\mapsto p(f)} is said to be \df{invariant} to left translation %the action of \m{G} on \m{X} 
if \m{p(f)=p(f^t)} for any \m{f\in L(G)} and any \m{t\in G}. 
A set \m{P=\cbr{\seq{p}{k}}} of such invariants is said to be \df{complete} if 
\m{p_1(f)\<=p_1(f'),\:\ldots,\: p_k(f)\<=p_k(f')} implies \m{f'=f^t} for some \m{t\in G}. 
The objective of this paper is to find an efficiently computable yet complete set of invariant functionals. 

\subsection{The Fourier transform}

The \marginpar{Fourier transform} \df{Fourier transform} of a function \m{f\in L(G)} is the collection of matrices 
\begin{equation*}
  \h f(\rho)=\sum_{x \in G} \rho(x)\, f(x) \qqquad\qqquad \rho\in\Rcal.  
\end{equation*}
With respect to the norms 
\begin{equation*}
  \nm{f}^2=\ovr{\abs{G}} \sum_{x\in G}\abs{f(x)}^2 
  \qquad\text{and}\qquad
  \nmbig{\h f}^2=\ovr{\abs{G}^2}\sum_{\rho\in\Rcal} d_\rho \nmbig{\h f(\rho)}_{2}^2, 
\end{equation*}
(where for an \m{n\times n} matrix \m{M},~ 
\m{\nm{M}_2=\brbig{\sum_{i,j=1}^n \sqb{M}_{i,j}}^{1/2}}~)
the transform \m{\mathfrak{F}\colon f\mapsto\h f} is unitary, and its inverse is given by 
%and the inverse transform is given by 
\begin{equation*}
  f(x)=\ovr{\abs{G}} \sum_{\rho\in\Rcal} d_\rho\: \tr\brbig{\rho(x) \cdot \h f(\rho)} \qqquad \qqquad x\in G. 
\end{equation*}
%From among the many special properties satisified by this transform, we will need the convolution 
Defining the \df{convolution} of two functions \m{f,g\in L(G)} as 
\begin{equation*}
  \br{f\ast g}(x)=\sum_{y\in G} f(xy^{-1})\: g(y),
\end{equation*}
it is easy to verify that %see that the Fourier transform obeys 
the convolution theorem \m{\widehat{f \ast g}(\rho)=\h f(\rho) \cdot \h g(\rho)} holds. 
Another property of interest   
is the behavior of the Fourier transform under translation: 
%Given \m{f\in L(G)} and a group element \m{g\tin G}, 
%The \df{left-translate} of \m{f} is 
%the function %\m{f^z\in L(G)} defined 
%\m{f^z(x)=f(z^{-1} x)}. 
%Then 
\begin{equation}\label{eq: translation}
  \h {f^t}(\rho)=\sum_{x \in G} \rho(x)\, f(t^{-1}x)
  =\sum_{x \in G} \rho(tx)\, f(x)
  =\rho(t)\sum_{x \in G} \rho(x)\, f(x)
  =\rho(t)\cdot \h f(\rho). 
\end{equation}
%hence, left translation by \m{z} has the effect of multiplying \m{\h f(\rho)} on the left by \m{\rho(z)}. 
Finally, if we define \m{f^{-1}\in L(G)} as \m{f^{-1}(x)=f(x^{-1})}, 
then \m{\h {f^{-1}}(\rho)=\h f(\rho)^\dag}.  
%for all \m{\rho}. 

In \marginpar{covariance}
general, we say that a matrix-valued functional \m{F\colon L(G) \to \CC^{D \times d_\rho}} is \m{\rho}-\df{covariant} 
if \m{F(f^t)=\rho(z)\cdot  F(f)} for any \m{f\in L(X)} and any \m{t\in G}. 
Similarly, \m{F'\colon L(X) \to \CC^{d_\rho\times d_\rho}} is \m{\rho}-\df{contravariant} if 
\m{F'(f^t)=F'(f)\cdot \rho(t)^\dag}. 
Clearly, the adjoint (conjugate transpose) of a \m{\rho}-covariant functional is \m{\rho}-contravariant. 
%, in particular, \m{\h f(\rho)^\dag} are \m{\rho}-contravariant. 
%Denoting complex conjugation by~\m{{}^\ast} and the Hermitian adjoint %of a matrix \m{M} by 
%\m{{M^\ast}^\top} by \m{M^\dag}, 
%by unitarity, \m{{\h f^\dag (\rho)}} is \m{\rho}-{contravariant}. 

\subsection{The power spectrum}

If \marginpar{spectrum} 
\m{F} is \m{\rho}-covariant and \m{F'} is \m{\rho}-contravariant, then %by unitarity %each matrix entry of the product   
\m{Q(f)=F'(f)\: F(f)} is invariant, i.e., \m{Q(f^t)=Q(f)}. 
%then \m{Q(f^g)=F'(f) \rho^{-1}(g) \rho(g) F(f)=Q(g)}, hence every matrix element of \m{Q} 
%is invariant to the action of \m{G} on \m{X}. 
Thus, %as \m{\rho} ranges over \m{\Rcal},  
the matrices \m{\h q(\rho)=\h f(\rho)^\dagger \: \h f(\rho)} are a natural starting point for finding 
left-invariant functionals. 
On reflection, this is not surprising, since \m{\h q\:} 
% it is not surprising that \m{\br{\h q(\rho)}_{\rho\in\Rcal}} is invariant, since it 
%Observe that \m{\h q(\rho)} 
is the Fourier transform of the \df{autocorrelation} 
\begin{equation*}
  q(x)=
        \sum_{y\in G} f^{-1}(xy^{-1})\,f(y)=
        \sum_{y\in G} f(yx^{-1})\,f(y)= 
        \sum_{y\in G} f(y)\,f(yx),  
\end{equation*}
%where \m{\mbox{}^\ast} denotes complex conjugation. 
which is manifestly invariant to left-translation of \m{f}. 
We call \m{\br{\h q(\rho)}_{\rho\in\Rcal}} the \df{spectrum} of \m{f}. 

%However, the elements of \m{\h q(\rho)} are 
Unfortunately, the matrix elements of \m{\br{\h q(\rho)}_{\rho\in\Rcal}} 
fall short of forming a complete set of invariants.  % functionals, 
This is because the spectrum is insensitive to the relative 
``phase'' of the various Fourier components.  
%For this we have to look at higher order spectra. 
%The \df{triple correlation} of \m{f} is defined  
It is natural to then look at higher order spectra. 

\subsection{Triple correlation and the bispectrum}

Recall \marginpar{Clebsch-Gordan}
that for any \m{\rho_1 \rho_2\in\Rcal}, the tensor product representation 
\m{\rho_1\otimes \rho_2} decomposes into irreducible components in the form 
\begin{equation}\label{eq: deco1}
  (\rho_1 \otimes \rho_2)(x)=
  \rho_1(x)\otimes \rho_2(x)=
  C_{\rho_1\rho_2}\,
  \sqbbigg{\:\bigoplus_{\rho\in\Rcal} \rho(x)^{\oplus m_\rho}\:}\:  C_{\rho_1\rho_2}^\dag, 
\end{equation}
where \m{C_{\rho_1\rho_2}} is a unitary matrix called the \df{Clebsch-Gordan} matrix, 
\m{m_\rho=m(\rho_1,\rho_2,\rho)} is the multiplicity of \m{\rho}, and 
\m{M^{\oplus k}} is a shorthand for \m{\bigoplus_{i=1}^k M}.  

Now \marginpar{bispectrum} 
consider the tensor product of the Fourier matrices \m{\h f(\rho_1)} and \m{\h f(\rho_2)}. 
Under translation 
\begin{equation*}
  \h f(\rho_1)\otimes \h f(\rho_2)\quad \mapsto\quad  
  \h {f^t}(\rho_1)\otimes \h {f^t}(\rho_2)=
  \br{\rho_1(t)\otimes \rho_2(t)} \cdot \brN{\h f(\rho_1)\otimes \h f(\rho_2)}, 
\end{equation*}
hence
\begin{equation*}
  C_{\rho_1\rho_2}^\dag\ts \brbig{\h {f^t}(\rho_1)\otimes \h {f^t}(\rho_2)}\, C_{\rho_1\rho_2} =
 \sqbbigg{\:\bigoplus_{\rho\in\Rcal} \rho(t)^{\oplus m_\rho}\:}~
  C_{\rho_1\rho_2}^\dag\ts \brbig{\h f(\rho_1)\otimes \h f(\rho_2)}\, C_{\rho_1\rho_2}.    
\end{equation*}
% \m{\h f(\rho_1)\otimes \h f(\rho_2)} 
%\m{C_{\rho_1\rho_2} ^\dag \brN{\h f(\rho_1)\otimes \h f(\rho_2)}\, C_{\rho_1\rho_2}} 
%which shows that \m{C_{\rho_1\rho_2}^\dag\ts \brbig{\h f(\rho_1)\otimes \h f(\rho_2)}\, C_{\rho_1\rho_2}} 
%splits into \m{\rho}-covariant sets of columns. % according to \rf{eq: deco1}. 
We may say that \m{C_{\rho_1\rho_2}^\dag\ts \brbig{\h {f}(\rho_1)\otimes \h {f}(\rho_2)}\, C_{\rho_1\rho_2}} 
is \m{\bigoplus_\rho \rho^{\oplus m_\rho}}-invariant. 
%In particular, multiplying \m{C_{\rho_1\rho_2} ^\dag \brN{\h f^\dag (\rho_1)\otimes \h f^\dag (\rho_2)}\, C_{\rho_1\rho_2}} 
%on the right by a direct sum of Fourier transform matrices according to the same scheme as in \rf{eq: deco1}, 
%gives an invariant matrix.  
%Hence, the matrices %as \m{\rho_1} and \m{\rho_2} range over \m{\Rcal}, 
In particular, 
%multiplying it on the left by \m{\bigoplus_\rho {\h f(\rho)^\dag}\mbox{}^{\oplus m_\rho}} 
%gives an invariant matrix. 
%The \df{bispectrum} is just a slightly rearranged version of this construction: 
the \df{bispectrum}  
\begin{equation}\label{eq: bispectrum}
  \h b(\rho_1,\rho_2)=\brBig{\h f(\rho_1) \otimes \h f(\rho_2)}^\dag\:
  C_{\rho_1\rho_2}\:
  \sqbbigg{\:\bigoplus_{\rho\in\Rcal} {\h f(\rho)}^{\oplus m_\rho} \:}\:  C_{\rho_1\rho_2}^\dag 
\end{equation}
is invariant to left-translations of \m{f}. 
%called the \df{bispectrum} of \m{f} gives furthe invariant functionals. 
%Another way to regard \m{\h q} is as the 
%\m{\br{\h q(\rho_1,\rho_2)}_{\rho_1,\rho_2\in\Rcal}} is none other than the 
%Fourier transform on the direct product group \m{G\times G}
%Recall that the elements of \m{G\times G} are pairs \m{(x_1,x_2)}, where \m{x_1,x_2\in G}. 
%We also use the fact from 
%of the \df{triple correlation}
%\begin{equation}\label{eq: triple corr}
%  q(x_1,x_2)=\sum_{y} f(y x_1)\,f(y x_2)\, f(y)^\ast.  
%\end{equation}
%Recall from general representation theory that the irreducible representations of \m{G\times G} are the tensor product representations 
%\m{\wbar{\rho}(x_1,x_2)=\rho_1(x_1)\otimes\rho_2(x_2)} with \m{\rho_1,\rho_2\in\Rcal}.
%which is a function defined on the direct product group \m{G\times G}
%\footnote{From general theory we know that the irreducible representations of \m{G\times G} are the tensor product representations 
%\m{\wbar{\rho}(x_1,x_2)=\rho_1(x_1)\otimes\rho_2(x_2)} with \m{\rho_1,\rho_2\in\Rcal}.}. 
The remarkable fact proved by Kakarala for compact groups in general is that 
provided that all \m{\h f(\rho)} are invertible, the matrix elements of the bispectrum are not only invariant, 
but also complete: there is no need to look at even higher order spectra 
\footnote{Kakarala defines the bispectrum in a slightly different form, equivalent to \rf{eq: bispectrum} up to 
unitary transforms and complex conjugation.}. 
%order correlations beyond the triple correlation.   
%Unfortunately, 

It is natural to ask what the analog of the autocorrelation is, i.e., what the invariant function is that the bispectrum is 
the Fourier transform of. 
For this we have to consider functions on the direct product group \m{G\times G}. 
Recall from general representation theory that the irreducible representations of %the product group 
\m{G\times G} are tensor product representations of the form  
\m{\rho_1(x_1)\otimes\rho_2(x_2)}, where \m{\rho_1,\rho_2\in\Rcal}.  
In particular, 
\begin{equation*}
  \h f(\rho_1)\otimes\h f(\rho_2) =
        \sum_{x_1\in G} \sum_{x_2\in G} \br{\rho_1(x_1)\otimes \rho_2(x_2)} f(x_1)\ts f(x_2)
\end{equation*}
in \rf{eq: bispectrum} is the Fourier transform of \m{u(x_1,x_2)=f(x_1)\,f(x_2)}, 
while 
\begin{multline*}
    C_{\rho_1\rho_2}
  \sqbbigg{\:\bigoplus_{\rho\in\Rcal} {\h f(\rho)}^{\oplus m_\rho} \:}  C_{\rho_1\rho_2}^\dag = 
  \sum_{x\in G}   C_{\rho_1\rho_2}
  \sqbbigg{\:\bigoplus_{\rho\in\Rcal} {\h \rho(x)}^{\oplus m_\rho} \:}  C_{\rho_1\rho_2}^\dag\; f(x)=
  \\ \sum_{x\in G} \br{\rho_1(x)\otimes \rho_2(x)} f(x)
\end{multline*}
is the Fourier transform of 
\begin{equation*}
  v(x_1,x_2)=
  \begin{cases}
    ~~f(x_1)&\text{if } x_1=x_2\\
    ~~0&\text{otherwise}. 
  \end{cases}
\end{equation*}
Thus, by the convolution theorem (on \m{G\< \times G}), \rf{eq: bispectrum} is the Fourier transform of 
\m{u^{-1}\ast v}, where \m{u^{-1}(x_1,x_2)=u(x_1^{-1},x_2^{-1})}. 
In long hand, \m{\h b} is the Fourier transform of  
\begin{multline*}
  %a(x_1,x_2)=
  \sum_{y_1\in G}\sum_{y_2\in G} u^{-1}(x_1 y_1^{-1}\!, x_2 y_2^{-1})\, v(y_1,y_2)=
  \sum_{y_1\in G}\sum_{y_2\in G} u(y_1 x_1^{-1}\!,y_2 x_2^{-1})\, v(y_1,y_2)=\\
  \sum_{y\in G} u(y x_1^{-1},yx_2^{-1})\,f(y)=
  \sum_{y\in G} f(y x_1^{-1})\,f(y x_2^{-1})\,f(y).%=a(x_1^{-1},x_2^{-1}),        
\end{multline*}
The function 
\begin{equation}\label{eq: triple correlation}
  b(x_1,x_2)=\sum_{y\in G} f(y x_1^{-1})\,f(y x_2^{-1})\,f(y)
\end{equation}
%The right hand side of 
%The function \m{a\colon G\times G\to\CC} 
%\rf{eq: triple correlation} 
is known as the \df{triple correlation} of \m{f}. 
%Since by \rf{eq: triple correlation}, the bispectrum as defined in \rf{eq: bispectrum} 
Just as the bispectrum (and under the same conditions) the \m{\cbr{b(x_1,x_2)}_{x_1,x_2}} components  
furnish a complete set of left-invariant functionals of \m{f}. 
In fact, Kakarala derives the concept of bispectrum from the triple correlation, 
and not the other way round. 

\subsection{Computational considerations}

The price to pay for the completeness of the bipsectrum and the triple correlation is the inflation in the size of the data. 
Letting \m{\abs{G}} denote the cardinality of \m{G}, the triple correlation consists of 
\m{\abs{G}^2} scalars, and by unitarity the total number of entries in the bispectrum matrices is the same. 
The symmetry \m{b(x_1,x_2)=b(x_2,x_1)} and its counterpart \m{\h b(\rho_1,\rho_2)=\h b(\rho_2,\rho_1)} 
(up to reordering of rows and columns) 
reduces the number of components that would actually be computed to \m{\absG(\absG+1)/2}, 
but to simplify our analysis we ignore this improvement by a constant factor. 

The computational cost of calculating \rf{eq: triple correlation} directly is \m{\absG^3}. 
The cost of computing the bispectrum involves two factors: the cost of computing the Fourier transform, 
and the cost of multiplying the various matrices appearing in \rf{eq: bispectrum}. 

Recent years have seen the emergence of fast Foruier transforms for a series of non-commutative groups, 
including the symmetric group \cite{Clausen89}, wreath product groups, ... 
Typically these algorithms reduce the complexity of Fourier transformation from \m{O(\absG^2)} to 
\m{O(\absG \log \absG)}. 
While a general theorem stating that Fourier transformation on an arbitrary finite group is possible in 
\m{O(\absG \log \absG)} time has not been proven, this does appear to be a plausible conjecture, 
which we adopt as an assumption for the rest of this paper. 
Hence, Fourier transformation is not the dominant factor in the cost of computing the bispectrum.

To estimate the cost of the matrix multiplications, we use the well known general identity 
\m{\sum_{\rho\in\Rcal}d_\rho^2=\absG} (this can be regarded as a corollary of the fact that the Fourier 
transform is an invertible linear map). 
For simplicity we take the naive upper bound of \m{O(D^3)} as the complexity of multiplying \m{D}-dimensional matrices. 
The cost of the multiplications appearing in \rf{eq: bispectrum} is then \m{d_{\rho_1}^3 d_{\rho_2}^3}. 
As an aside we note that in practical applications the final 
multiplication by \m{C^\dag_{\rho_1,\rho_2}}  may be omitted, since this just effects a unitary transform. 
Summing over all \m{\rho_1,\rho_2\in\Rcal} and using the crude inequlity 
\m{\sum_{\rho\in\Rcal} d_{\rho}^3\leq \brbig{\sum_{\rho\in\Rcal}d_\rho^2} \brbig{\sum_{\rho\in\Rcal} d_\rho}
\leq \brbig{\sum_{\rho\in\Rcal}d_\rho^2} \brbig{\sum_{\rho\in\Rcal} d^2_\rho}=\absG^\theta} 
yields an overall complexity bound of \m{O(\absG^{2\theta})} for the bispectrum. 



==> backgroundFFT.tex <==
\section{Background: Clausen's FFT}





==> conclusions.tex <==
\section{Conclusions}

The bispectrum is an elegant way of constructing invariants of functions on finite groups with respect to 
translation, but from a computational point of view it is not necessarily attractive. 
We discussed the theory behind the bispectrum from a new angle, and arrived at a unitarily equivalent set of invariants,  
which we named the skew spectrum. 
Not only is the skew spectrum easier to compute, it also meshes naturally with the structure of 
Clausen-type fast Fourier transforms, promising efficient specialized algorithms for 
computing it on specific groups or homogeneous spaces of groups.  


==> homo2.tex <==
\subsection{Homogeneous spaces}


==> invariants.tex <==
\section{The skew spectrum}

Notwithstanding their elegance, 
the computational demands of both the 
triple correlation %\rf{eq: triple correlation} 
and the bispectrum %\rf{eq: bispectrum} 
are of serious concern in practical applications. 
The former involves an explicit convolution over \m{G}, while %leading to a total computational cost of \m{\abs{G}^3}. 
the latter circumvents convolution, at the expense of multiplying together large matrices and 
requiring Clebsch Gordan matrices. In this section we derive a third, unitarily equivalent set of invariants, 
which strike the middle ground. 

Our starting point is to decompose the triple correlation into \m{\abs{G}} separate functions. % over \m{G}. 
Specifically, given \m{g\colon G\times G\to\CC} and some member \m{z} of \m{G},  
we define the \df{left \m{z}-diagonal slice} 
and the \df{right \m{z}-diagonal slice} of \m{g} as respectively 
%of \m{g} as %the function \m{g_z\colon G\to \CC} 
\begin{equation*}
  g\Lslice{z}(x)=g(x,zx) 
  \qqquad \text{and} \qqquad 
  g\Rslice{z}(x)=g(x,xz).%\qqquad x\in G. 
\end{equation*}
Now we define \m{r_z\colon G\to \CC} as 
\begin{equation*}
  r_z(x)=u\Rslice{z}(x)=f(x)\, f(xz).
\end{equation*}
Clearly, the Fourier components of these functions are \m{\rho}-covariant, since  
\begin{equation*}
  \h r^{t}_z(\rho)= 
  \sum_{x \in G} \rho(x)\, f(t^{-1}x)\, f(t^{-1}x z)
  =\sum_{x \in G} \rho(tx)\, f(x)\,f(xz)
  %=\rho(t)\sum_{x \in G} \rho(x)\, f(x)
  =\rho(t)\cdot \h r_z(\rho). 
\end{equation*}
This immediately gives rise to the left-translation invariant matrices 
\begin{equation}\label{eq: skew spectrum}
  \h q_z(\rho)=\h r_z(\rho)^\dag\cdot \h f(\rho) \qqquad\rho\in\Rcal, 
\end{equation}
which we collectively call the \df{skew spectrum} of \m{f}.
 
%To see that up to unitary transformation these matrices again embody same invariants as the bispectrum and the triple correlation 
To see that the skew spectrum and the bispectrum are unitarily equivalent, 
observe that by the convolution theorem 
\begin{multline*}
  q_z(x)=\sum_{y\in G} r^{-1}_z(x y^{-1})\, f(y)
  =\sum_{y\in G} r_z(y x^{-1})\, f(y)\\
  =\sum_{y\in G} f(y x^{-1})\,f(y x^{-1}\nts z)\, f(y)
  =b(x,z^{-1} x)
  =b\Lslice{z^{-1}}(y),  
\end{multline*}
and that \m{\cbr{b\Lslice{z^{-1}}\,}_{z\in G}} together make up the entire triple correlation. 
We thus have the following theorem. 

\begin{thm}
  Let \m{f} and \m{f'} be complex valued functions on a finite group \m{G}, 
  with a complete set of inequivalent irreducible representations \m{\Rcal}. 
  %and let \m{\h f} and \m{\h f'} 
  %be their respective Fourier transforms with respect to some complete set \m{\Rcal} of inequivalent irreducible 
  %representations of \m{G}. 
  Assume that \m{\h f(\rho)} is invertible for all \m{\rho\in\Rcal}.  
  Let the skew spectrum \m{\h q_z} be defined as in \rf{eq: skew spectrum}. 
  %Now let \m{\h q_z} and \m{\h q'_z} be the diagonal bispectra 
  %Now let \m{\h r_z} be the Fourier transform of \m{r_z(x)=f(x)f(xz)}, and let 
  %\m{\h q_z(\rho)=\h r_z(\rho)^\dag \cdot \h f(\rho)} be the diagonal bispectrum. 
  %Define \m{\h q'_z(\rho)} analogously. 
  Then \m{f'=f^t} for some \m{t\in G} if and only if \m{\h q'_z(\rho)=\h q_z(\rho)} for all \m{z\in G} and all \m{\rho\in\Rcal}. 
\end{thm}

From a computational perspective, the skew spectrum involves \m{\abs{G}+1} independent Fourier transforms followed by 
\m{\abs{G}} sequences of multiplying \m{\cbr{\CC^{d_\rho\times d_\rho}}_{\rho\in\Rcal}} matrices. 
By similar considerations to those in the previous section, the cost of the former is \m{O(\absG^2 \log \absG)}, 
while the cost of the latter is \m{O(\absG^{\theta+1})}, improving slightly on both the triple correlation and the bispectrum.  
The more substantial advantages of the skew spectrum become apprent when restricting to  functions on  
homogeneous spaces of \m{G}.  



==> symm.tex <==
\section{The symmetric group}\label{sec: symm}

The symmetric group serves as a good example of the techniques developed in the previous sections. 
Recall that the symmetric group over \m{n} letters, denoted \m{\Sn}, is the group formed by the set of 
bijective maps (permutations)  
\m{\sigma\colon \cbr{\oneton{n}}\to\cbr{\oneton{n}}} under composition. 

The irreducible representations of \m{\Sn} are indexed by partitions of \m{n}, by which me mean 
weakly decreasing sequences of positive integers \m{\lambda_1\geq\lambda_2\geq\ldots\geq\lambda_k} 
satisfying \m{\sum_{i=1}^k\lambda_i=n}. 
This is denoted \m{\lambda\vdash n}, where \m{\lambda=\br{\seq{\lambda}{k}}}. 
Integer partitions are represented graphically by Young diagrams, which consist of laying 
down \m{\seq{\lambda}{k}} boxes in consecutive rows. As an example, the diagram 
\begin{equation*}
  \yng(4,2,2)
\end{equation*}
corresponds to the \m{(4,2,2)} partition and indexes an irreducible representation of \m{\Sbb_8}. 

Functions on \m{\Sn} often arise in practical problems in the context of rankings. 
For example, in a social survey \m{f(\sigma)} might be the number of respondents 
who rank candidate \m{\sigma(1)} first, candidate \m{\sigma(2)} second, etc.. 
Diaconis discusses a whole series of problems in this vein \cite{Diaconis}. 
Left invariant functionals enter when trying to decide whether two such ranking functions \m{f} and \m{f'} on \m{\Sn} 
may be the same, given that between \m{f} and \m{f'} the candidates might have been permuted amongst themselves. 
This is a non-trivial problem because testing for all \m{n!} possible permutations is clearly very expensive. 





